EDEN Survey: Small Transiting Planet Detection Limits and Constraints on the Occurrence Rates for Late M Dwarfs within 15 pc

Earth-sized exoplanets that transit nearby, late spectral type red dwarfs will be prime targets for atmospheric characterization in the coming decade. Such systems, however, are difficult to find via wide-field transit surveys like Kepler or TESS. Consequently, the presence of such transiting planets is unexplored and the occurrence rates of short-period Earth-sized planets around late M dwarfs remain poorly constrained. Here, we present the deepest photometric monitoring campaign of 22 nearby late M dwarf stars, using data from over 500 nights on seven 1-2 meter class telescopes. Our survey includes all known single quiescent northern late M dwarfs within 15 pc. We use transit-injection-and-recovery tests to quantify the completeness of our survey, successfully identify most ($>80\%$) transiting short-period (0.5-1 d) super-Earths ($R > 1.9 R_\oplus$), and are sensitive ($\sim50\%$) to transiting Earth-sized planets ($1.0-1.2 R_\oplus$). Our high sensitivity to transits with a near-zero false positive rate demonstrates an efficient survey strategy. Our survey does not yield a transiting planet detection, yet it provides the most sensitive upper limits on transiting planets orbiting our target stars. Finally, we explore multiple hypotheses about the occurrence rates of short-period planets (from Earth-sized planets to giant planets) around late M dwarfs. We show, for example, that giant planets at short periods ($<1$ day) are uncommon around our target stars. Our dataset provides some insight into occurrence rates of short-period planets around TRAPPIST-1-like stars, and our results can help test planetary formation and system evolution models, as well as guide future observations of nearby late M dwarfs.

==> revisions/referee_report.tex <==
=================[ REFEREE'S COMMENT]========================
The authors present observations of 22 M7-L0 dwarfs within 15 pc. These objects were targeted as part of the EDEN survey, which uses a network of seven longitudinally distributed 0.8 - 2.3-m telescopes to enable continuous monitoring of targets in order to search for planetary transits (under ideal observing conditions). These spectral types represent a largely unexplored parameter space for transiting exoplanets. Detecting more of these planets would be valuable for a number of reasons, including the possibilities of follow-up atmospheric characterization and of informing planet formation models around very-low-mass objects.

Each object was targeted for at least 25 hours, and for most stars in the sample, this dataset represents the highest quality photometric monitoring to date. The data were searched for transiting planets and candidate signals were identified in the light curves of EIC 9. Follow-up observations of this target yielded no repeat transit events. A planet injection/recovery simulation was performed using the data, resulting in the following inferences:
1) The fraction of late-M dwarfs hosting TRAPPIST-1 b analogs, full TRAPPIST-1-like systems, and giant planets on 1-day periods cannot be constrained to less than 100% with the current data set.
2) The fraction of late-M dwarfs with giant planets on 0.5-day periods can be constrained with an upper limit of 75% at 95% confidence.

Accept/Revise/Reject Decision
I unfortunately have to recommend that the paper be rejected on the grounds that it does not contain significant new results. I appreciate the amount of work that went into obtaining and analyzing the observations, but the reported occurrence rate constraints do not represent an improvement compared to previous studies. For example, the 75% upper limit on late-M dwarfs with giant planets on 0.5-day periods is less constraining than results from Sestovic & Demory (2020) and Sagear et al. (2020) who searched for planets around similar spectral types in K2 data. Additionally, the injection/recovery of TRAPPIST-1-b and full TRAPPIST-1 analogs are unable to place any constraint on the occurrence rates of such systems.

I have left a number of major and minor comments below that, if addressed, would make the paper a stronger candidate for acceptance in the future. Fundamentally, however, I think that more targets need to be observed in order to actually achieve tighter constraints on planet occurrence rates around late-M and early-L dwarfs.

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee's detailed review and comments. We believe that we have addressed every comment stated below, and in our response we detail how we address the referee's comments. The revised manuscript shows these changes in bold-faced text.

=================[ REFEREE'S COMMENT]========================

Section 3: I think that it's critically important to have some discussion of the effects of time-variable precipitable water vapor (PWV) on the photometry. The GC495 filter used by EDEN overlaps a number of water vapor bands which can produce percent-level changes on short timescales. I suggest quantifying the effects that PWV has in the GC495 filter. The difference between the expected integrated counts from an EDEN target and from comparison stars can be quantified by convolving sky models with different levels of PWV, model source spectra, the filter profile, and the quantum efficiency curve of one of the survey's CCDs. I think this is especially important because reference star spectral types are not accounted for in creating the median-combined reference light curve that detrends the target flux.

-----------[ AUTHORS' RESPONSE]========================
This is a very good point. At this time we do not have the methodology in place to model and correct for precipitable water vapor (PWV) at our telescope sites. However, as was shown in several studies and as the referee pointed out, the potential source of error is too large to be ignored. We added a new subsection in Section 3 where we discuss precipitable water vapor and acknowledge its relevance for our setup and choice of filters, as well as further evaluation/correction steps we would perform upon a potential candidate detection surviving initial vetting. 

We further cannot exclude PWV as a source for the singular unexplained, transit-like event we saw in data from the Kuiper telescope. We thus add PWV as a potential source to the discussion in Sect. 7.2.

=================[ REFEREE'S COMMENT]========================

Sections 4.1/4.2: There needs to be more discussion of the criteria that are used to consider an injected planet as "detected". Does the period identified by TLS need to be within some percent of the true period? Are period aliases considered in the identification step?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and have added a paragraph in Section 4.2, after where we first discuss the injection and recovery process, that states our boundaries on the detection of injected planets both in percentage of true period and undersampled periods due to scarcity of our data.

=================[ REFEREE'S COMMENT]========================

Figure 4:
Binned photometry with error bars should be shown along with the raw photometry to more clearly reveal trends.
The same parameters in the same panels in each plot.
Each panel should be described in the caption, along with what is denoted by the green and black-dashed lines.
The three transit events should all be shown with an accurate manual flag. It's difficult at first glance to identify them otherwise, especially in the first plot.
Since all subplots are shown with the same x-range, it would make sense to reformat as a 5x1 plot instead of the 3x2 format that it has now. This would make it easier to compare the auxiliary features with the target light curve.
The x/y ranges in each panel should be restricted to minimize white space.
A corrected light curve should be shown in each plot with the median trend divided out.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and have made the following changes to the figure:
- Added errorbars and 10-minute binned photometry to every plot
- Described the figure a bit better in the caption
- Put in an accurate manual flag for each figure
- Removed the auxiliary features as we couldn't get all of them to show up properly for each data set
- The data has already been median filtered

=================[ REFEREE'S COMMENT]========================

Section 6:
"First, we constrained the occurrence rate of TRAPPIST-1 b analogs and TRAPPIST-1-like planetary systems." The occurrence rates of these planets have not been constrained with the current data set, and this is acknowledged in the Summary. I think the abstract ("Our dataset provides insight into the short-period planet population around TRAPPIST-1-like host stars...") should be edited to reflect this.
"Second, we constrained the occurrence rate of close-in (P < 1 day) giant planets." It was found that less than 75% of late M dwarfs host a giant planet on 0.5-day orbital periods at 95% confidence. Unfortunately, I don't think that this is a new constraint. Sestovic & Demory (2020) found a cumulative occurrence rate of less than ~15% for planets larger than Neptune to 95% confidence around similar spectral types. Similar results were seen in Sagear et al. (2020).

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this detailed comment and have addressed it in the following manner.
- We changed the abstract to say "Our dataset provides some additional insight into the occurrence rate of short-period planets specifically around TRAPPIST-1-like host stars"
- We changed the verb "constrained" to "analyzed" in the end of Section 6 Paragraph 1.
- We added in a paragraph with an upper limit analysis in the similar vein to Sagear et al. (2020).

=================[ REFEREE'S COMMENT]========================

Lines 67-68 - "Arguably, the best-suited planets for in-depth spectroscopic studies..." Does this mean the best terrestrial planets, specifically?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this clarification and have added that we mean terrestrial planets.

=================[ REFEREE'S COMMENT]========================

Lines 75-77 - "...limiting the feasibility of transit observations to systems that are very close to us" Limiting the feasibility of transit spectroscopy, not of transit observations.

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee and made the above change.

=================[ REFEREE'S COMMENT]========================

Lines 93-100 - I disagree that ground-based transit surveys like MEarth, SPECULOOS, and PINES have revealed the increase in small planet occurrence rates for early M dwarfs. I would argue that this information has come primarily from the Kepler mission, and it will be supplemented by TESS as the mission progresses (see, e.g., Brady & Bean 2022). Occurrence rate studies have also been published with CARMENES and HADES data (Sabotta et al. 2021 and Pinamonti et al. 2022, respectively), but with far fewer detections than Kepler.

The ground-based transit surveys, like EDEN, perform star-by-star searches for individual exoplanet systems, and are not suited for developing a population-level understanding of planets across the M spectral class. This can be seen in the number of discoveries from each of these projects so far: MEarth - 3; SPECULOOS - 1 (or 2, if you count TRAPPIST-1); PINES - 0. Compare these to the dozens of detections from the RV surveys, and hundreds from the space-based transit surveys.

Another issue with referencing these various projects as revealing the increase in small planet occurrence rates around early M dwarfs is that they probe different spectral types. Generally speaking, Kepler data is sensitive to planet detection out to early M spectral types, while TESS, CARMENES, and HADES are sensitive out to mid M's. SPECULOOS covers late-M to late-L dwarfs, while PINES doesn't target M dwarfs at all, having a sample that exclusively consists of L and T dwarfs. I suggest that the introduction be reworded to account for these facts.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this comment and have adjusted our introduction to account for the different spectral types for the ground based surveys and included information from Kepler, K2, and TESS. However, we also state that these surveys under-represent the M-dwarf population and are biased towards the larger and brighter M dwarfs, so these targeted and volume-limited ground-based surveys of late-M dwarfs will still provide the least biased constraints on planet occurrence rates near the substellar boundary.

=================[ REFEREE'S COMMENT]========================

Lines 102-108 - "Hardegree-Ullman et al. (2019) revealed..." The Hardegree-Ullman results do not show a significant increase in planet occurrence rates for mid-M's compared to early M's. The SNR of the difference between their measured occurrence rate for mid-M dwarfs (1.19_(-0.49)^(+0.70)) versus those for early M dwarfs from Dressing & Charbonneau (2015) (0.63_(-0.06)^(+0.08)) is only about 1.1. I would say that their results show a tentative increase in short-period planet occurrence rates for mid-M dwarfs.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this comment and have adjusted the wording slightly to include the numbers and the phrase "evidence for a higher occurrence rate"

=================[ REFEREE'S COMMENT]========================

Lines 111-112 - "...provide feedback to planet formation models." Which models? They should be reference here.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for pointing this out and have added many planet formation model population references.

=================[ REFEREE'S COMMENT]========================

Lines 116-117 - "...targeting, in particular, planetary systems within 15 pc." I suggest rewording, since EDEN is searching for planets, not targeting known planetary systems. Maybe "targeting the detection, in particular...".

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee's suggestion and have made the appropriate revision.

=================[ REFEREE'S COMMENT]========================

Lines 276-277 - "...Tables 1 and 2.2." This sentence should refer to Table 2, not 2.2.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for finding this typo and have fixed it.

=================[ REFEREE'S COMMENT]========================

Lines 277-278 - "As the completeness of our targets within 15 pc increased during the survey..." This wording is confusing to me, why did the increase in completeness of targets within 15 pc prompt an extension of the sample out to 21 pc?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this clarification, and we have updated the text to denote that we observed stars outside the 15 pc volume as secondary targets when our main candidate stars were either observed to an acceptable level and/or seasonally unavailable for observation.

=================[ REFEREE'S COMMENT]========================

Lines 292-294 - "This step is coded to be optional in cases of bad or unavailable calibration files." How often is this the case? Is the light curve quality significantly affected when flats/biases are not used?

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee bringing this clarification to our attention and have added text to address this, stating this occurs less than 5% of the time and that there is no real significant change to the light curve quality when flats and biases are not used.

=================[ REFEREE'S COMMENT]========================

Lines 294-296 - "Next, we calculated an astrometric solution using astrometry.net and photutils." How is photutils used to calculate the astrometric solution? Isn't that just returned directly from astrometry.net?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for the question and have updated the text to reflect that we calculate the astrometry as part of calculating the photometry, so astrometry.net is used as part of the photutils photometric solution.

=================[ REFEREE'S COMMENT]========================

Lines 297-298 - "...selecting the aperture size between 5-50 pixels..." In what size steps? One pixel as in Gibbs et al. (2020)?

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee's question and have included the clarification of one pixel steps for the aperture (as in Gibbs et al. 2020).

=================[ REFEREE'S COMMENT]========================

Lines 380-383 - "...as well as those signals with low false alarm probabilities but with parameters that are not physically motivated: transit durations < 15 minutes, orbital periods < 0.25 days, transit depths corresponding to planets < 0.1R_Earth." I think the wording is confusing here, because these requirements are not non-physical (i.e., you can certainly have transit durations < 15 minutes, periods < 0.25 days, or sizes < 0.1 R_Earth). Are these cuts intended to discourage models that the data is not likely to have actually detected?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and have reflected this in the text, stating that these cuts are intended to discourage transit models of planets that are extremely unlikely to exist as well as to be found in our data.

=================[ REFEREE'S COMMENT]========================

Lines 410-413 - "We created 250 planets with a random orbital period, orbital phase, and planet radius within each of the given grid bins..." Was an impact parameter of 0 assumed, or was it randomly assigned between 0-1 (or 0-1+R_p)? Were circular orbits assumed? What limb darkening law/coefficients were assumed?

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee for pointing this out and have included this information in the paper: impact parameter was randomly assigned between 0 and 0.7 to avoid grazing partial transits, orbits assumed to be circular, and Claret (1998) limb-darkening with u1=0.84 and u2=0.125 was used.

=================[ REFEREE'S COMMENT]========================

Line 437 - "...studies of stellar activity..." - I suggest citing Lin et al. (2021) and Murray et al. (2022) here.

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee and have added citations to these studies.

=================[ REFEREE'S COMMENT]========================

Caption of Figure 2 - "...it is such a strong signal." I agree, but the strength of this signal should be quantified. The SNR of the transit can be approximated as:
SNR≈(mean(flux[out-of-transit])-mean(flux[in-transit]))/√(σ[out-of-transit]^2+σ[in-transit]^2 ) ,
where σis the standard deviation.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and have added the strength of the signal to the calculation.

=================[ REFEREE'S COMMENT]========================

Caption of Figure 3 - "The inner edge of the HZ is defined using the Kopparapu et al. (2013) model based on the temperature and insolation." What stellar effective temperature and what planetary albedo was assumed for calculating the insolation?

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee pointing this out and have updated the caption to include the stellar effective temperature of 2600 K and albedo of 0.3.

=================[ REFEREE'S COMMENT]========================

Line 545 - "...(P=1.511 days) and planet radius (R=1.116 R_Earth)..." Please cite these values.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for noticing this and have added the proper citation.

=================[ REFEREE'S COMMENT]========================

Lines 561-562 - "...and a Rayleigh distribution for mutual inclinations around 2 deg." This seems like a high value to me, as Luger et al. (2017) ("Planet-Planet Occultations in TRAPPIST-1...") measured a mutual alignment of planets in the TRAPPIST-1 system of less than 0.3 deg. I don't think adopting this value would strongly impact the conclusions of the simulation, but I suggest citing the Luger paper.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this clarification and have added the citation to the Luger paper and a short explanation.

=================[ REFEREE'S COMMENT]========================

Lines 568-569 - "...and in 79% of the surveys we would not have detected any planets in the sample." For consistency with the conclusions of the previous paragraph, I would instead describe this result in the positive: "we would have detected at least one planet in 21% of the simulated surveys."

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee and have made the suggested change.

=================[ REFEREE'S COMMENT]========================

Line 613 - "utilizes" --> "utilized", as MEarth is no longer active.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and implemented it.

=================[ REFEREE'S COMMENT]========================

Caption of Figure 5 - "transit-like features are visible" --> "a transit-like feature is visible."

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee and have made the suggested change.

=================[ REFEREE'S COMMENT]========================

Lines 719-720 - "...only one strong transit candidate." I would be careful with the wording here, as in the previous section it was concluded that this target is not a strong transit candidate.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion and have updated the text to refer specifically to the single transit that remained instead of the candidate.

==> revisions/referee_report_2.tex <==
=================[ REFEREE'S COMMENT]========================
I thank the authors for their revised draft, which I think is much improved over the first submission. However, I think that moderate revisions are still required before the paper is suitable for publication. As before, they are split into major and minor comments.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for their suggestions in both rounds of the revision and agree with all of the comments, with the changes as follows.

=================[ REFEREE'S COMMENT]========================
Major Comments
1) Figure 4:
a. I am principally confused by the identified transit event in the top panel. To my eye, there is no clear pre-/post-transit baseline where the purported transit has been marked, certainly nothing as clear as in the second and third panels. Since the event is also not seen in the detrended data, I think this light curve should be excluded from Figure 4 and the analysis in Section 7.2.
b. The panels have titles that read "LSPM_J0149+4233 on at (telescope)". Presumably the date should be listed in the titles between "on" and "at".
c. It's stated in the text that the LOT/Kuiper features were both ~45 minutes in duration, whereas the VATT feature was ~1 hour. For the sake of comparing the timescales of transit features, I recommend that all three panels be shown on the same x range.
d. Otherwise, I think this figure is greatly improved from the first submission!

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for this detailed comment and have addressed it as follows:
a) We agree that there is nothing clear in the transits for the detrended data, but there has been some processing applied in the new panel for this figure, and then additional detrending for the next figure. However, we do want to include the light curve showing that there was something that caught our eye there, because the main reason we followed up on the target was the LOT and VATT first-look "features" matching the TESS period within minutes. To do this, we added another figure showing the first-look light curves (taken from the original form of this figure in the first submission) and then added text to highlight the differences between this light curve and the more processed versions.
b) We have remade the titles so that the date is showing up correctly.
c) We have stretched the three images so that the time scales are identical.

=================[ REFEREE'S COMMENT]========================
2) Section 7.2:
a. More details are needed on the light curves of EIC 9 with candidate transit events: What were the weather conditions on the nights of the candidate transit events? Were there clouds? Do the target and reference centroids during the candidate transit events look okay?
b. I think it is necessary to at least qualitatively estimate whether or not the ~1% transit depth seen in the detrended Kuiper light curve can be achieved with reasonable levels of PWV variability. I expect that the GG495 filter has a similar PWV response to the I+z' filter used by SPECULOOS since they have similar overlap of NIR water vapor bands. Referring to Figure 7 from Murray et al. (2020) or Figure 2 from Pederson et al. (2023), you can see that changes of only a few mm in PWV can cause a second-order extinction effect of over 1% in I+z'-band (depending on the spectral types of your reference stars), which could potentially explain the transit event in the Kuiper light curve. At the minimum, these two references should be cited in the second-to-last paragraph of this section. It would be useful to see the second-order extinction effect evaluated in the GG495 filter in the future, but I understand that this is probably beyond the scope of this work.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for this comment and have added in text to address the weather conditions on the nights of the observations and the guiding of the telescopes, as well as a paragraph on the PWV variability typical for the Kuiper telescope location. We agree that the GG495 extinction effect is beyond the scope of this work.

=================[ REFEREE'S COMMENT]========================
3) Figure 6:
a. Are the expected mid-transit times in this figure calculated using the TESS period of 2.883 days? If so, why are the expected times for Lulin (Taiwan) and Kuiper (Arizona) within ~1 hour of each other, when they were both observed on 2020-11-18?
b. Why is 2019 data from the Bok telescope mentioned in the text but not shown in the figure?

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing this out and have adjusted the text to state that the Calar Alto and Lulin mid-times were based on the TESS period while the Kuiper is based on a 2.886-day period instead, and have also expanded on the fact that the Bok data was not able to rule out the transit due to high scatter in the light curve.

=================[ REFEREE'S COMMENT]========================
4) Figures 7-9:
a. Why are the detection fractions for 2MASS J0351-0052 and 2MASS J1534-1418 so low compared to the other targets? They seem to be two extreme outliers compared to the other 22 targets. Would their exclusion from your analysis improve your occurrence rate map? I suspect that this would not have a very significant impact, but it would be worth at least discussing why these two targets have sensitivity maps that are so different from the others in Section 5.3.
b. It looks like the inner edge of the HZ is in the same location for each sensitivity map, matching its location in Figure 3 and 4 (i.e., assuming a T_eff of 2600 and an albedo of 0.3). I think its position in Figures 7-9 should be calculated for each target individually, since you have the spectral type of each target.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for these comments and have added a paragraph to Section 5.3 detailing how these two have an unfortunate combination of relatively low total observation time, southern declination, and relatively high individual light curve scatter, but that keeping them does not significantly affect our occurrence rate map. We have also gone through and updated each of the individual figures with the inner HZ edge for each star.

=================[ REFEREE'S COMMENT]========================
Minor Comments
1) Lines 261 - 262: "...there is no introduction of a systematic error." --> "...there is no introduction of a systematic error by their removal."

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee on adding this suggested text and have made this adjustment.

=================[ REFEREE'S COMMENT]========================
2) Line 301: "...implemented a correction factor..." Eq. 4 from Furlan et al. (2014) indicates that it is for correcting a planet radius around a binary star, but the text never states explicitly that a candidate transit was found around EIC 14. I don't think this correction factor is worth mentioning here, but you could add it to Section 4.1, explaining that you account for the dilution of potential transit depths around EIC 10 and 14 by implementing a correction factor following Eq. 4 from Furlan et al. (2014).

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee on the proposed change and have moved the discussion of the correction factor to Section 4.1, with only a pointer to the info in Section 2.2.

=================[ REFEREE'S COMMENT]========================
3) Line 458: "...likely to exist..." --> "...unlikely to exist..."?

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing this out and have made the suggested change.

=================[ REFEREE'S COMMENT]========================
4) Lines 633 - 634: "...mini-Neptune planets just greater than 1 day." --> "...mini-Neptune planets with orbital periods just greater than 1 day." This should also be fixed in the caption of Figure 4.

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee that the suggested wording is clearer and have edited the text accordingly.

=================[ REFEREE'S COMMENT]========================
5) Line 764: "...we identified a transit-like feature on EIC 9..." --> "...we identified transit-like features in light curves of EIC 9, with depths of ~0.5-1% and a duration of ~45 minutes."

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee on this suggestion and have adjusted the text.

=================[ REFEREE'S COMMENT]========================
6) Lines 1037 - 1050: The Author Contributions section is cut off.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing this out and have fixed it in our new revision.
